Street TryOn: Learning In-the-Wild Virtual Try-On from Unpaired Person Images

Most virtual try-on research is motivated to serve the fashion business by generating images to demonstrate garments on studio models at a lower cost. However, virtual try-on should be a broader application that also allows customers to visualize garments on themselves using their own casual photos, known as in-the-wild try-on. Unfortunately, the existing methods, which achieve plausible results for studio try-on settings, perform poorly in the in-the-wild context. This is because these methods often require paired images (garment images paired with images of people wearing the same garment) for training. While such paired data is easy to collect from shopping websites for studio settings, it is difficult to obtain for in-the-wild scenes. In this work, we fill the gap by (1) introducing a StreetTryOn benchmark to support in-the-wild virtual try-on applications and (2) proposing a novel method to learn virtual try-on from a set of in-the-wild person images directly without requiring paired data. We tackle the unique challenges, including warping garments to more diverse human poses and rendering more complex backgrounds faithfully, by a novel DensePose warping correction method combined with diffusion-based conditional inpainting. Our experiments show competitive performance for standard studio try-on tasks and SOTA performance for street try-on and cross-domain try-on tasks.

==> sec/sup_datasets.tex <==
To build a benchmark for street try-on, we collect street fashion images from fashion retrival dataset DeepFashion2~\cite{}.
The DeepFashion2 dataset releases a total of 191,961 images for the training set and 32,153 images for the validation set. These images feature models wearing an assortment of clothing items belonging to 13 popular clothing categories. For each image, a comprehensive set of annotations is available, encompassing information on scale, occlusion, zoom-in level, viewpoint, category, style, bounding box coordinates, dense landmarks, and per-pixel masks. 

To meet the specific requirements of our research, a three-stage data filtering process was employed for both the training and validation datasets. In the initial stage, filtering was performed based on DeepFashion2's annotation data to select images featuring models with a frontal view, minimal occlusion, absence of excessive zoom-in, and images originating from professional sources, such as shops or merchants. This initial filtering process leveraged the annotations provided for``viewpoint,"``occlusion," ``zoomIn," and ``shop" on each image to make the necessary selections. 
Subsequently, in the second stage of filtering, the focus was on identifying images that portrayed the entire upper body or full body of the models. Keypoint detection was utilized for this purpose, Specifically, the alpha pose algorithm was applied to the complete set of validation and training images to extract keypoint coordinates. Images were kept if the keypoint coordinates for the "Left Shoulder," "Right Shoulder," "Left Hip," and "Right Hip" were present. Additionally, human parsing annotations were utilized to classify image pixels into various categories. If any pixels were classified under the "face" and "top-wear" categories , the image was included, while the rest were discarded.
 
 Following these two stages of meticulous filtering, the dataset was refined to encompass a total of 12,364 images for the training set and 2,089 images for the validation set. This final dataset comprises professional images of models in frontal view, devoid of substantial occlusion or watermarks, exhibiting the appropriate scale (absence of excessive zoom-in), and featuring the complete upper body.
Furthermore, in an effort to enhance the quality of annotations for the validation images, a manual inspection process was undertaken. Among the 2,089 validation images in the final dataset, specific attributes were manually assessed and labeled, including the presence of the full body, frontal view, arms positioned across garments, substantial occlusion on the torso, the presence of a crossbody bag, the presence of text or print, the presence of a jacket, the presence of a long skirt or dress, the existence of watermarks on the image, the presence of padding on the image, and the modeling pose of sitting.






==> tables/ablation_bg_remove_backup.tex <==
\begin{table}[!htb]
\centering \small
\vspace{-3mm}
\caption{\small Comparison on street2street's foregronud and background. FS-VTON, SDAFN and HR-VTON are {\bf retrained} for model2model tryon with DeepFashion data. PASTAGAN++'s official release is used which is trained for model2model. Street2street try-on for segmented foreground try-on only (FG-tryon), foreground try-on blended with inpainted background (FG-tryon + BG inpainted), and running inference for each model without foreground segmentation (end-to-end). }
\vspace{-3mm}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|c||c c  c |}
\hline
       & \makecell{FG-tryon only \\ (w/o BG)} & \makecell{FG tryon + \\ BG inpainted} & \makecell{end-to-end \\ (w/ BG)}  \\ \hline
FS-VTON     & 35.137     & 53.018    & 67.009   \\
HR-VITON    & 41.154     & 55.857    & 63.539   \\
SDAFN       & 34.274     & 47.634    & 42.436   \\
PASTAGAN++  & 36.267      & 49.732   & 67.016 \\ \hline
Ours         & \textbf{31.218}  &     \textbf{46.178}   & \textbf{33.039}   \\
\hline
\end{tabular}
}
\label{tab:background_removal}
\end{table}

\begin{table}
	\begin{minipage}{0.4\linewidth}
		\caption{Caption }
		\label{tab:le}
		\centering
		\resizebox{\textwidth}{!}{%
		\begin{tabular}{|c||c c  c |}
\hline
       & \makecell{FG-tryon only \\ (w/o BG)} & \makecell{FG tryon + \\ BG inpainted} & \makecell{end-to-end \\ (w/ BG)}  \\ \hline
FS-VTON     & 35.137     & 53.018    & 67.009   \\
HR-VITON    & 41.154     & 55.857    & 63.539   \\
SDAFN       & 34.274     & 47.634    & 42.436   \\
PASTAGAN++  & 36.267      & 49.732   & 67.016 \\ \hline
Ours         & \textbf{31.218}  &     \textbf{46.178}   & \textbf{33.039}   \\
\hline
\end{tabular}
	\end{minipage}\hfill
	\begin{minipage}{0.6\linewidth}
		\centering
		\captionof{figure}{Caption_2}
		\label{figu:re}
		\includegraphics[width=0.8\textwidth]{Figs/Pair1.PNG}
	\end{minipage}
\end{table}


==> tables/ablation_diffusion_old.tex <==
\begin{table}[!htb]
\centering
\caption{Ablation}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|cc||c c c|c|c|c|}
\hline
\multirow{2}*{Warping} & \multirow{2}*{Fusion}   & \multicolumn{3}{c|}{Shop2Shop} & Shop2Str  & M2Str  & Str2Str \\ 
& & SSIM & FID & LPIPS & FID \\ \hline
FS-VTON & FS-VTON & 0.883 & 9.552 & 0.091 & 90.972 & 80.288 &  74.120 \\
FS-VTON & SD-inpaint &  &   &   &    \\
ours & FS-VTON &  & 12.544   &  &  64.046 & 71.512 & 72.408 \\
ours & SD-inpaint & 0.840 & 9.671  & 0.113  &  \textbf{33.819} & \textbf{34.050} & \textbf{33.165} \\

\hline

\end{tabular}
}

\label{tab:vitonhd_table}
\end{table}

==> tables/ablation_robustness.tex <==




\begin{figure}
\vspace{-5mm}
\centering

\begin{minipage}{0.7\textwidth}
\centering
      \includegraphics[width=\textwidth]{figures/ablation_warping_vs_diffusion.pdf} 
      %\subcaption{Visual Results.}

\end{minipage}
%\vspace{-5mm}
\begin{minipage}[c]{\textwidth}
%\vspace{-240px}
%\hspace{90px}
\centering
\resizebox{0.7\textwidth}{!}{

    \begin{tabular}[t]{|cc||c|}
        \hline
        Warping Method & Fusion Method  & Shop2Street (FID)  \\ \hline
        FS-VTON & FS-VTON & 90.972 \\
        FS-VTON & SD-inpainting & 77.456 \\
        ours & FS-VTON &   64.046 \\
        ours & SD-inpainting &  \textbf{33.819} \\
        \hline
    \end{tabular}
    }
    \vspace{-3mm}
\end{minipage}

\caption{
Comparison with warping and compositing (fusion) modules of FS-VITON~\cite{he2022styleflow} in FID. 
%We use the officially released model weights for both components of FS-VTON in all the experiments at 256x192. 
\textbf{Top:} Visual Results.
\textbf{Bottom:} Quantitative Results. 
 \label{fig:ablation_robustness}
 }

\end{figure}
 %\vspace{-5mm}

==> tables/ablation_robustness_backup.tex <==




\begin{figure}
\centering
\floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=0.5\textwidth}}]{figure}[]{
     \caption{Comparison with warping and compositing (fusion) modules of FS-VITON in FID. We compare each component with FS-VTON~\cite{he2022styleflow} at 256$\times$192, at which are modules of FS-VTON are trained. We use the officially released model weights for both components of FS-VTON in all the experiments. (a) Quantitative Results. (b) Visual Results. \label{fig:ablation_robustness}}

    
 }{
\subfloat[]{
\resizebox{0.5\textwidth}{!}{
    \begin{tabular}[t]{|cc||c|}
        \hline
        Warping Method & Fusion Method  & Shop2Street (FID)  \\ \hline
        FS-VTON & FS-VTON & 90.972 \\
        FS-VTON & SD-inpainting & 77.456 \\
        ours & FS-VTON &   64.046 \\
        ours & SD-inpainting &  \textbf{33.819} \\
        \hline
    \end{tabular}
    }
}

\subfloat[]{	
    \includegraphics[width=0.5\textwidth]{figures/ablation_warping_vs_diffusion.pdf}
}

 }
\end{figure}


==> tables/benchmark_attribute.tex <==
\begin{table*}[!htb]
\centering
\caption{Virtual Try-On Benchmarks}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c c c c|c c c c|}
\hline
    Method & paired  & person src  & garment src & category & Shop2Model  & Shop2Street & Model2Street & Street2Street \\ \hline
     
VITON 
& \checkmark & model & shop & top 
& \checkmark & $\times$ & $\times$ & $\times$
\\
VITON-HD \cite{choi2021vitonhd}
& \checkmark & model & shop & top 
& \checkmark & $\times$ & $\times$ & $\times$
\\

DressCode
& \checkmark & model & shop & top,bottom,dress 
& \checkmark & $\times$ & $\times$ & $\times$
\\

UPT
& $\times$ & model & model & top,bottom,dress 
& \checkmark & $\times$ & $\times$ & $\times$
\\
\hline
ours
& $\times$ & model,street & shop, model, street & top,bottom,dress 
& \checkmark & \checkmark & \checkmark & \checkmark
\\
\hline


\end{tabular}
}

\label{tab:benchmark_table}
\end{table*}

==> tables/complex_exp.tex <==
\begin{table*}[!htb]
\centering
\caption{
\textbf{Comparsions with prior work in same-domain and cross-domain tests.} 
%Test ``A2B'' means the garment from source A is going to be tried on by a person from source B.
For Shop2Model (VITON-HD test), we compare with numbers shared by the authors of GP-VTON~\cite{xie2023gp-vton}, who re-trained all prior work on VITON-HD at 512$\times$384. For Shop2Street, we use the released models trained at 256$\times$192 resolution, and evaluate at the same resolution. For the remaining tests, we use the officially released models to compare at 512$\times$320, where PWS\cite{albahar2021posewithstyle} results are first generated at its native resolution of 512$\times$352 and then resized to 512$\times$320. GP-VTON requires fine-grained human parse labeled manually or detected by non-released estimator, which is not applicable to our street person images.
Note, PWS is trained on DeepFashion~\cite{liu2016deepfashion}, and PASTAGAN++ is trained on UPT dataset~\cite{xie2021pastagan}, where both are model2model datasets. PASTAGAN++ (street) is trained from scratch on the proposed Street TryOn dataset.
}
\vspace{-3mm}
\resizebox{\textwidth}{!}{

\begin{tabular}{|c||ccc||ccc|c||c|c|c|}
\hline
\multirow{5}*{}
     & \multicolumn{3}{c||}{Training Settings}
     & \multicolumn{3}{c|}{Shop2Model (VITON-HD)}
     & Shop2Street
     & Model2Model
     & Model2Street
     & Street2Street \\ 
     & \small{paired}
     & \small{garment src}
     & \small{person src}
      & \small{FID $\downarrow$}
      & \small{SSIM $\uparrow$} 
      & \small{LPIPS $\downarrow$} 
     & \small{FID $\downarrow$}
     & \small{FID $\downarrow$} 
     & \small{FID $\downarrow$}
     & \small{FID $\downarrow$}
     \\\hline
     
PFAFN~\cite{ge2021pfafn} 
& \checkmark & shop & model 
& 9.475 & 0.886 & 0.087
& 97.597
& \textcolor{blue}{@chang - retrain?}
&  \textcolor{blue}{@chang - eval?}
& \textcolor{blue}{@chang - eval?}
\\ 

FS-VTON~\cite{he2022styleflow} 
& \checkmark & shop & model 
& 9.552 & 0.883 & 0.091
& 90.972
& 13.926
& \textcolor{red}{@aiyu - eval}
& 67.009 
\\ 

HR-VITON~\cite{lee2022hrvton} 
& \checkmark & shop & model 
& 0.862 & 16.21  & 0.109
&  \textcolor{red}{@aiyu - eval}
& 20.404
& \textcolor{red}{@aiyu - eval}
& 63.539 
\\ 

SDAFN~\cite{bai2022sdafn} 
& \checkmark & shop & model 
& 9.400 & 0.882 & 0.092
& 106.036
& 14.316
& \textcolor{green}{@jay - eval}
& 42.432 
\\ 


GP-VTON~\cite{xie2023gp-vton} 
& \checkmark & shop & model 
 & \textbf{9.197} & \textbf{0.894} & \textbf{0.080}
& n.a.
& n.a.
& n.a.
& n.a. 
\\

StableVITON~\cite{xie2023gp-vton} 
& \checkmark & shop & model 
 & \textcolor{blue}{@chang - eval?} & \textcolor{blue}{@chang?} & \textcolor{blue}{@chang?}
& 37.211
& \textcolor{blue}{@chang - retrain?}
& \textcolor{blue}{@chang - eval?}
& \textcolor{blue}{@chang?}
\\ \hline

%DiOr~\cite{dior} 
%& paired & model & model 
%& - & - & - 
%& -
%& \textcolor{red}{@aiyu}
%& \textcolor{red}{@aiyu}
%\\ 

PWS~\cite{albahar2021posewithstyle} 
& \checkmark & model & model 
& - & - & - & - 
& 34.224
& 76.889
& 84.326
\\ 


PastaGAN++~\cite{xie2022pastagan++} 
& $\times$ & model & model  
& - & - & - & - 
& 13.848
& 71.090
& 67.016 \\

PastaGAN++ (street)
& $\times$ & street & street  
& - & - & - & - 
& 40.841
& 70.461
& 67.088

\\ \hline

%ours (w/o SD)
%& paired & shop & model 
%%&  &  & 
%%& 64.046 & 71.512 & 72.408
%%\\ 

ours (1)
& \checkmark & shop & model 
& 9.671 & 0.840 & 0.113
& \textbf{33.819} 
& 10.961
& \textbf{34.050} & 33.165
\\ 

ours (2)
& $\times$ & model & model 
& 11.675 & 0.826 & 0.128
&35.135 & 11.040 & 34.434 & 33.742 \\ 

ours (3)
& $\times$ & street & street  
&11.951 & 0.823 & 0.129
& 34.054 & \textbf{10.214} & 34.191 & \textbf{33.039}
 \\
\hline

\end{tabular}
}


\label{tab:main_result_table}
\end{table*}

==> tables/original_ablation_study.tex <==
\begin{table*}[!htb]
\centering

\caption{Ablation Study.}

\begin{tabular}{|c||cc|c|c|c|}
\hline
\multirow{2}*{}
     & \multicolumn{2}{c|}{Street2Street} 
     & Model2Street
     & Shop2Street
     & Shop2Shop (VITON-HD) \\ 
     & \small{Dress} 
     & \small{Top} 
     & \small{Top} 
     & \small{Top}  
     & \small{Top}  
     \\\hline
     
(A) Baseline
& 100.587
& 59.665
& 59.732
& 62.247
& 54.482

\\\hline

(B) +DP. warp 
& 38.974
& 34.853
& 34.412
& 36.319
& 22.942
\\\hline

(C) + DP. warp + Undressing
& \textbf{34.115}
& 34.012
& 34.218
& \textbf{35.371}
& 14.028

\\\hline

(D) + DP. warp + Undressing + Warp cor. 
& 34.747
& \textbf{33.043}
& \textbf{34.197}
& 35.636
&
\\\hline

\end{tabular}

\label{tab:ablation_table}
\end{table*}

==> tables/person2person_table.tex <==
\begin{table*}[!htb]
\centering
\caption{
\textbf{Evaluation on Street2Street, Model2Street, and Model2Model tests.} 
%Test ``A2B'' means the garment from source A is going to be tried on by a person from source B.
We retrain FS-VTON, HR-VTON and SD-VTON on DeepFashion dataset for Model2Model try-on at 512$\times$320. For the remaining tests, we use the officially released models to compare at 512$\times$320, where PWS\cite{albahar2021posewithstyle} results are first generated at its native resolution of 512$\times$352 and then resized to 512$\times$320. %GP-VTON requires fine-grained human parse labeled manually or detected by non-released estimator, which is not applicable to our street person images.
Note, PWS is trained on DeepFashion~\cite{liu2016deepfashion}, and PASTAGAN++ is trained on UPT dataset~\cite{xie2021pastagan}, which are both Model2Model datasets. PASTAGAN++ (street) is trained from scratch on the proposed Street TryOn dataset.
}
\vspace{-3mm}
\resizebox{\textwidth}{!}{

\begin{tabular}{|l||ccc||c|c|c|}
\hline
\multirow{5}*{}
     & \multicolumn{3}{c||}{Training Settings}
     
     & Street2Street 
     & Model2Street
     & Model2Model
     \\ 
    \raisebox{1.5ex}[0ex][0ex]{Methods} & \small{paired}
     & \small{garment src}
     & \small{person src}
      
     & \small{FID $\downarrow$} 
     & \small{FID $\downarrow$}
     & \small{FID $\downarrow$}
     \\\hline
     
%ours (w/o SD)
%& paired & shop & model 
%%&  &  & 
%%& 64.046 & 71.512 & 72.408
%%\\ 

Ours (Paired, VITON-HD)
& \checkmark & shop & model 
& 33.165
& \textbf{34.050} 
& 10.961
\\ 

Ours (Unpaired, VITON-HD)
& $\times$ & model & model 
& 33.742 & 34.434 & 11.040  \\ 

Ours (Unpaired, StreetTryOn)
& $\times$ & street & street  
& \textbf{33.039} & 34.191  & \textbf{10.214}
 \\
\hline


FS-VTON~\cite{he2022styleflow} 
& \checkmark & model & model 
& 67.009 
& 77.273
& 13.926
\\ 

HR-VITON~\cite{lee2022hrvton} 
& \checkmark & model & model 
& 63.539 
& 55.172
& 20.404
\\ 

SDAFN~\cite{bai2022sdafn} 
& \checkmark & model & model 
& 42.432 
& 44.537
& 14.316
\\ 


PWS~\cite{albahar2021posewithstyle} 
& \checkmark & model & model 
& 84.326
& 76.889
& 34.224
\\ 


PastaGAN++~\cite{xie2022pastagan++} 
& $\times$ & model & model  
& 67.016 
& 71.090
& 13.848
\\

PastaGAN++ (street)
& $\times$ & street & street  
& 67.088
& 70.461
& 40.841

\\ \hline


\end{tabular}
}


\label{tab:person2person_table}
\end{table*}

==> tables/shop2person_table.tex <==
\begin{table*}[!htb]
\centering
\caption{
\textbf{\small Evaluation on Shop2Street and Shop2Model tests.} 
%Test ``A2B'' means the garment from source A is going to be tried on by a person from source B.
For Shop2Model, we compare with numbers shared by the authors of GP-VTON~\cite{xie2023gp-vton}, who re-trained all prior work on VITON-HD at 512$\times$384. For Shop2Street, we use the released models trained at 256$\times$192 resolution for PFAFN, FS-VTON, and evaluate at the same resolution, and resize output images to 256$\times$192 for comparison for these methods with released models at higher resolution.
}
\vspace{-3mm}
\resizebox{\textwidth}{!}{

\begin{tabular}{|l||ccc||c|ccc|}
\hline
\multirow{5}*{}
     & \multicolumn{3}{c||}{Training Settings}
    
     & Shop2Street 
      & \multicolumn{3}{c|}{Shop2Model (VITON-HD)} \\ 
    \raisebox{1.5ex}[0ex][0ex]{Methods} & \small{paired}
     & \small{garment src}
     & \small{person src}
      
     & \small{FID $\downarrow$}
     & \small{FID $\downarrow$}
      & \small{SSIM $\uparrow$} 
      & \small{LPIPS $\downarrow$} 
     \\\hline


%ours (w/o SD)
%& paired & shop & model 
%%&  &  & 
%%& 64.046 & 71.512 & 72.408
%%\\ 

Ours (Paired, VITON-HD)
& \checkmark & shop & model 
& \textbf{33.819} 
& 9.671 & 0.840 & 0.113

\\ 

Ours (Unpaired, VITON-HD)
& $\times$ & model & model 
&35.135 
& 11.675 & 0.826 & 0.128
 \\ 

Ours (Unpaired, StreetTryOn)
& $\times$ & street & street  
& 34.054 
&11.951 & 0.823 & 0.129
\\ \hline
     
%PFAFN~\cite{ge2021pfafn} 
%& \checkmark & shop & model 
%& 97.597
%& 9.475 & 0.886 & 0.087
%\\ 

SDAFN~\cite{bai2022sdafn} 
& \checkmark & shop & model 
& 106.036
& 9.400 & 0.882 & 0.092

\\ 

FS-VTON~\cite{he2022styleflow} 
& \checkmark & shop & model 
& 90.972
& 9.552 & 0.883 & 0.091

\\ 

HR-VITON~\cite{lee2022hrvton} 
& \checkmark & shop & model 
& 63.516
& 16.21  & 0.862  & 0.109

\\ 




GP-VTON~\cite{xie2023gp-vton} 
& \checkmark & shop & model
& n.a.
% & \textbf{9.197} & \textbf{0.894} & \textbf{0.080}
 & 9.197 & 0.894 & 0.080

\\

StableVITON~\cite{kim2023stableviton} 
& \checkmark & shop & model 
& 35.883
 & \textbf{8.233} & \textbf{0.888} & \textbf{0.073}

\\ \hline





\end{tabular}
}


\label{tab:shop2person_table}
\end{table*}

==> tables/street_tryon_benchmark_stats.tex <==
\begin{table}[!htb]
\centering

\caption{The proposed Benchmark tests.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{|c|c| c c| c|}
\hline
    Test & type & garment src & person src  & \# pairs \\ \hline\hline
     
\multirow{2}*{street2street} & dress & street & street & 1,190 \\
& top & street & street & 909 \\ \hline
model2street & top & VITON-HD person & street & 909 \\\hline
shop2street & top & VITON-HD garment & street & 909 \\\hline
shop2model & top & VITON-HD garment & VITON-HD person & 2,032 \\
\hline

\end{tabular}
}

\label{tab:street_tryon_benchmark_stats}
\end{table}

==> tables/upt_and_street_table.tex <==
\begin{table*}[!htb]
\centering
\begin{tabular}{|c||cc||cc|cc|cc|cc|}
\hline
\multirow{2}*{}
     & \multicolumn{2}{|c||}{Street Try-On} 
     & \multicolumn{2}{c|}{UPT (upper-clothes)} 
     & \multicolumn{2}{c|}{UPT (lower-clothes)} 
     & \multicolumn{2}{c|}{UPT (upper-and-lower)}  
     & \multicolumn{2}{c|}{UPT (dresses)}  \\ 
     \hline
     & FID $\downarrow$ & HE. $\uparrow$ 
     & FID $\downarrow$ & HE. $\uparrow$ 
     & FID $\downarrow$ & HE. $\uparrow$ 
     & FID $\downarrow$ & HE. $\uparrow$ 
     & FID $\downarrow$ & HE. $\uparrow$ \\\hline
     
PBAFN~\cite{pbafn} 
& n.a. &   -  
& 11.79 &   - 
& n.a. &   - 
& n.a. &   - 
& n.a. &   - \\ 

DiOr~\cite{dior} 
& n.a. &   -  
& 25.87 &   - 
& 28.17 &   - 
& 26.24 &   - 
& 54.11 &   - \\ 

wFlow~\cite{wflow} 
& n.a. &   -  
& 14.30 &   - 
& 14.17 &   - 
& 16.36 &   - 
& 34.81 &   - \\ 

PWS~\cite{albahar2021posewithstyle} 
& n.a. &   -  
& 11.15 &   - 
& 13.29 &   - 
& 12.60 &   - 
& 28.44 &   - \\ 

PASTAGAN~\cite{xie2021pastagan} 
&   n.a.    &   -  
&   6.69    &
&   8.65    &
&   9.51    & 
&   32.03   & \\ 

PASTAGAN++
& \textcolor{red}{Viraj} &   -  
&   5.65    &
&   7.40    & 
&   8.20    & 
&   22.89   & \\ \hline

Ours
& - &   -  
& - &   - 
& - &   - 
& - &   - 
& - &   - \\

\hline

\end{tabular}


\label{tab:upt_table}
\end{table*}
